CRPlace: Camera-Radar Fusion with BEV Representation for Place Recognition

The integration of complementary characteristics from camera and radar data has emerged as an effective approach in 3D object detection. However, such fusion-based methods remain unexplored for place recognition, an equally important task for autonomous systems. Given that place recognition relies on the similarity between a query scene and the corresponding candidate scene, the stationary background of a scene is expected to play a crucial role in the task. As such, current well-designed camera-radar fusion methods for 3D object detection can hardly take effect in place recognition because they mainly focus on dynamic foreground objects. In this paper, a background-attentive camera-radar fusion-based method, named CRPlace, is proposed to generate background-attentive global descriptors from multi-view images and radar point clouds for accurate place recognition. To extract stationary background features effectively, we design an adaptive module that generates the background-attentive mask by utilizing the camera BEV feature and radar dynamic points. With the guidance of a background mask, we devise a bidirectional cross-attention-based spatial fusion strategy to facilitate comprehensive spatial interaction between the background information of the camera BEV feature and the radar BEV feature. As the first camera-radar fusion-based place recognition network, CRPlace has been evaluated thoroughly on the nuScenes dataset. The results show that our algorithm outperforms a variety of baseline methods across a comprehensive set of metrics (recall@1 reaches 91.2%).

==> sec/backup.tex <==

% \begin{figure}[htbp]
% % \begin{figure}[t]
% \centering
% {\includegraphics[width=0.5\textwidth]{figs/challengev5.png}}
% \caption{Comparison between the baseline place recognition method and our BACRPlace. (a) Challenge posed by visual degradation. Previous method retrieves a incorrect candidate for a query in a rainy condition. (b) Challenge posed by dynamic objects. Place recognition retrieves a false negative candidate due to the misleading of dynamic objects. Our camera-radar fusion-based Place recognition method is able to address these challenges.}
% \label{challenge}
% \end{figure}
% \section{Introduction}

% Global localization plays a crucial role in autonomous driving by addressing the fundamental question of ``where am I within a predefined reference map''. Place recognition is an essential component of global localization since it is able to retrieve a place within a large map database that closely matches the current place. In particular, it plays a vital role in Simultaneous Localization and Mapping (SLAM), aiding in the detection of loop closures to rectify drift and tracking errors. 

% %An example is shown in Figure \ref{challenge} (a), the state-of-the-art visual place recognition \cite{xu2023leveraging} fails to retrieve the correct candidates in a rainy condition. 
% Visual place recognition \cite{arandjelovic2016netvlad, radenovic2018fine, berton2022rethinking, khaliq2022multires, hausler2021patch} has been widely studied due to the low cost and rich texture information provided by cameras. However, visual place recognition still faces three main challenges. First, previous visual place recognition methods use single-view image to extract global descriptor, which fail to retrieve the correct candidates when revisiting the same place from different perspectives, as shown in Figure \ref{challenge} (a). In other words, rotation invariance is not considered. Bird's Eye View (BEV) representation has a natural advantage in achieving rotation invariance. Second, it is easily affected by visual degradation such as rain, snow, and direct sunlight, see Figure \ref{challenge} (b). Third, existing methods have not taken into account the impact of dynamic objects on place recognition. Since place recognition relies primarily on scene similarity, dynamic objects could be misleading due to landmark inconsistency, as shown in Figure \ref{challenge} (c). Therefore, it is necessary to extract global descriptors that focus on stationary background information while ignoring dynamic objects. 

% To address the first challenge, a recent work, called vDiSCO \cite{xu2023leveraging}, has proposes a method to employ BEV representation for 360-degree visual place recognition, achieving remarkable results. The authors extract BEV features from multi-view images based on BEVFormer \cite{li2022bevformer}, then combine the polar transformation and the Discrete Fourier transform to aggregate rotation-invariant global descriptors from BEV features, as shown in Figure \ref{baseline} (a). The second challenge can be improved by fusing camera and LiDAR sensors for place recognition. LiDAR-based place recognition methods \cite{uy2018pointnetvlad, chen2021overlapnet, xu2021disco, vidanapathirana2021locus, komorowski2021minkloc3d} offer improved robustness against illumination conditions and environmental changes but lack rich texture features. Camera-Lidar fusion-based methods \cite{lai2022adafusion, komorowski2021minkloc++, lee20232, pan2021coral, xu2023leveraging} combine the advantages of these two modalities, resulting in significant enhancements in performance and robustness. However, LiDAR is too expensive and susceptible to adverse weather conditions such as snow and fog. The third challenge has not been given due attention yet. As a result, millimeter-wave radar (referred to as radar in this paper) sensors are engaged because they are able to infer the object’s relative radial velocity based upon the Doppler effect, which can help us easily identify which objects are moving. More importantly, radar remains nearly unaffected by harsh weather conditions and obstacles. It is more lightweight and lower-cost than LiDAR. However, radar measurements are significantly noisier, sparser, lower-resolution and do not provide elevation compared to LiDAR, rendering LiDAR-based place recognition methods unsuitable for radar point clouds \cite{cai2022autoplace}. Although there have been efforts to exploit the unique characteristics of radar for place recognition \cite{suaftescu2020kidnapped, barnes2020under, cai2022autoplace}, how to effectively learn stationary background features while ignoring dynamic features by fully fusing the complementary characteristics of camera and radar remains a huge challenge. 
% % To provide a baseline for camera-radar fusion-based place recognition, we directly combine the feature extraction module of BEVFusion and the global descriptor aggregation module of vDiSCO, as shown in Figure \ref{baseline} (b). It also support camera-only and radar-only methods.
% Unlike camera and LiDAR, millimeter-wave radar (referred to as radar in this paper) remains nearly unaffected by harsh weather conditions and obstacles. It is more lightweight and lower-cost than LiDAR. However, due to the challenges of sparsity and noisy measurements in radar, it has become a popular practice to fuse camera and radar to exploit their complementary characteristics in 3D perception system. However, methods based on camera-radar fusion for the task of place recognition have not yet received any attention. In recent years, camera-radar fusion-based 3D object detection methods have been widely explored \cite{nabati2021centerfusion, kim2023craft, kim2023crn, lei2023hvdetfusion, pang2023transcar, kim2023rcm}. Unfortunately, these methods mainly focus on moving objects and ignore the background information, making it inappropriate to directly apply them to place recognition. Since place recognition relies primarily on scene similarity, dynamic objects could be misleading due to landmark inconsistency, as shown in Figure \ref{challenge} (b). Therefore, it is necessary to extract global descriptors that focus on stationary background information while ignoring dynamic objects. Although there have been efforts to exploit the unique characteristics of radar for place recognition \cite{suaftescu2020kidnapped, barnes2020under, cai2022autoplace}, how to effectively learn stationary background features while ignoring dynamic features by fully fusing the complementary characteristics of camera and radar remains a huge challenge. 

% In this work, we first provide a baseline for camera-radar fusion-based place recognition by directly combining the feature extraction module of BEVFusion \cite{liu2023bevfusion} and the global descriptor aggregation module of vDiSCO \cite{xu2023leveraging}. We will continue to refer to it as BEVFusion in this paper. It also support camera-only and radar-only methods. Further, we propose BACRPlace, a novel place recognition method that fully fuses the complementary characteristics of multi-view cameras and radars to generate background-attentive global descriptors. Specifically, BACRPlace first engages a Background-Attentive Bidirectional Fusion (BABF) strategy to focus on stationary background features while ignoring dynamic features. In our BABF strategy, a Background-Attentive Mask Generation (BAMG) module is first performed to create a background attention mask based on radar dynamic points. Then a Bidirectional cross attention-based Spatial Fusion (BSF) module is performed to enable thorough background feature interaction and adaptively learn the soft-association between camera BEV features and radar BEV features. 
% \begin{figure*}
%     \centering
%     \includegraphics[width=1\textwidth]{figs/baseline.png}
%     \caption{Baselines of the camera-radar fusion-based place recognition methods. (a) In vDiSCO, BEV features are extracted based on BEVFormer, and polar transform and DFT is combined to generate global descriptor for rotation invariance. (b) We develop a BEVFusion-based method to fuse camera and radar features for place recognition. (c) Global descriptor generation module of vDiSCO.}
%     \label{baseline}
% \end{figure*}

% In this work, we propose BACRPlace, a novel place recognition method that fully fuses the complementary characteristics of multi-view cameras and radars in the BEV representation to generate background-attentive global descriptors. Specifically, BACRPlace engages the Background-Attentive Bidirectional Fusion (BABF) strategy to focus on stationary background features while ignoring dynamic features. A Background-Attentive Mask Generation (BAMG) module is first engaged to create a background attention mask based on radar dynamic points. Then a bidirectional cross attention-based fusion module is performed to enable thorough background feature interaction and adaptively learn the soft-association between camera BEV features and radar BEV features. In summary, we make the following contributions:

% \begin{itemize}
% \item We propose a novel and robust Background-attentive Camera-Radar fusion-based place recognition method, namely BACRPlace, to combine the complementary characteristics of camera and radar in the BEV representation. To the best of our knowledge, this is the first work that fuses multi-view cameras and radars for the task of place recognition.  

% \item We propose an adaptive Background-Attentive mask generation method to explicitly supervise the network to learn stationary background features.

% \item We design a bidirectional attention-based fusion strategy to fully interact spatial features and adaptively learn the soft-association from two modalities. 

% \end{itemize}



